Behavior Change in Response to Subreddit Bans and External Events

As more people flock to social media to connect with others and form virtual communities, it is important to research how members of these groups interact to understand human behavior on the Web. In response to an increase in hate speech, harassment and other antisocial behaviors, many social media companies have implemented different content and user moderation policies. On Reddit, for example, communities, i.e, subreddits, are occasionally banned for violating these policies. We study the effect of these regulatory actions as well as when a community experiences a significant external event like a political election or a market crash. Overall, we find that most subreddit bans prompt a small, but statistically significant, number of active users to leave the platform; the effect of external events varies with the type of event. We conclude with a discussion on the effectiveness of the bans and wider implications for the online content moderation.

==> data/darknetmarkets/last_posting_date.tex <==



==> figs/darknetmarkets/dark_net_markets_active_users.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	3625	4081	4161
-19	3606	4098	4184
-18	3595	4112	4204
-17	3592	4131	4233
-16	3591	4153	4250
-15	3569	4169	4264
-14	3529	4169	4270
-13	3487	4165	4287
-12	3444	4165	4294
-11	3407	4154	4316
-10	3372	4131	4306
-9	3349	4120	4296
-8	3321	4118	4276
-7	3276	4103	4264
-6	3235	4080	4244
-5	3171	4051	4219
-4	3106	4012	4197
-3	3004	3965	4184
-2	2835	3929	4161
-1	2754	3892	4129
0	2720	3855	4113
1	2682	3820	4091
2	2614	3784	4070
3	2568	3754	4050
4	2538	3723	4032
5	2507	3705	4023
6	2480	3679	4002
7	2453	3658	3979
8	2427	3641	3962
9	2401	3620	3944
10	2360	3598	3927
11	2321	3561	3910
12	2289	3529	3888
13	2277	3508	3862
14	2255	3490	3843
15	2234	3457	3829
16	2210	3438	3806
17	2189	3419	3794
18	2176	3396	3776
19	2154	3380	3762
20	2137	3365	3745
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=DarkNetMarkets,
    clip=false,
    width=4cm,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}

==> figs/darknetmarkets/dark_net_markets_percentage_of_users_gone.tex <==
\begin{tikzpicture}
\begin{axis}[       
        ybar stacked,
        width=4cm,
        bar width=5pt, 
        title=DarkNetMarkets,
        xtick = {1,2,3,4,5,6,7,8,9,10},
        xticklabels = {$2^3$,$2^4$,$2^5$,$2^6$,$2^7$,Control,AskReddit},
        %yticklabels={1,300000}, 
]

%ALL OFF BY 2 FOR LOCATION PURPOSES

%1 week
\addplot+ coordinates
	{
(1,0.0189798339264531)
(2,0.0239234449760765)
(3,0.0297239915074309)
(4,0.0136054421768707)
(5,0.00942408376963355)
(6,0.00513321926179422)
};


%2 weeks
\addplot+ coordinates
	{
(1,0.0320284697508896)
(2,0.0406698564593301)
(3,0.0552016985138004)
(4,0.0340136054421769)
(5,0.0172774869109947)
(6,0.0100219995111219)
%(9,40)
%(10,6)
};


%3 weeks
\addplot+ coordinates
	{
(1,0.0403321470937129)
(2,0.0526315789473684)
(3,0.0636942675159235)
(4,0.0442176870748299)
(5,0.025392670157068)
(6,0.0144219017355169)
%(9, 7)
};


%4 weeks
\addplot+ coordinates
	{
(1,0.0498220640569394)
(2,0.0645933014354066)
(3,0.0764331210191082)
(4,0.0612244897959183)
(5,0.0301047120418848)
(6,0.0166218528477144)
%(9,27)
%(10,3)
};






\end{axis}
\end{tikzpicture}

==> figs/darknetmarkets/dark_net_markets_week_no_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	25.13587629	23.94641041	22.2333436
-19	25.32387396	23.92919466	22.51170468
-18	24.79700581	24.01709572	22.67706477
-17	24.37323391	23.6428431	21.74444554
-16	24.65710131	23.14307932	21.0200039
-15	24.83412188	23.78943857	21.87664143
-14	24.20910719	22.91449566	21.12501187
-13	24.66943522	23.17377449	21.34321755
-12	24.26518091	23.15990275	21.49227727
-11	24.44251997	22.74755219	21.57104408
-10	24.94279832	23.11205543	21.88492541
-9	23.59707743	22.50156682	20.97121711
-8	24.79904644	23.22894761	22.31836077
-7	24.27219771	22.91394928	22.07004616
-6	24.84091107	23.47088471	22.04497167
-5	24.74921657	23.17933899	20.99176918
-4	24.66063548	22.61264751	21.11624415
-3	24.46502602	23.03314967	21.2650634
-2	23.7629452	22.28820802	20.5265709
-1	23.79224326	23.06342743	21.16931818
0	22.26109391	23.15190463	21.06376445
1	23.63947676	23.82665522	21.29261782
2	22.79254189	22.6422205	20.59686061
3	23.001443	22.98681383	21.11704351
4	22.69761273	22.35206216	20.04710425
5	23.17127672	22.55745527	21.51688211
6	23.46218591	22.93673819	21.21826281
7	22.74396682	22.58333333	21.30189601
8	22.70753512	22.47416762	21.01571983
9	23.42268308	22.79036322	20.96983666
10	22.59955666	21.75185264	20.62110553
11	21.9128512	21.89056684	20.80066985
12	22.11708986	21.86703332	20.40143443
13	21.28064209	20.733847	19.59504219
14	22.26042916	22.10315627	20.73417722
15	22.47903139	21.86991511	20.43532129
16	22.01422957	21.94896598	20.45104895
17	21.96198871	21.40302013	20.47301182
18	22.33884525	21.46829434	20.73035158
19	22.20024773	21.71391549	20.42744597
20	21.84847645	21.64393339	20.48862173
}{\darknetmarkets}

==> figs/darknetmarkets/dark_net_markets_week_with_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	14.48882814	13.99387925	12.86991918
-19	14.90117661	14.17863085	13.37217732
-18	14.96101735	14.3591633	13.60785595
-17	14.76182553	14.29135964	13.08569052
-16	15.11397671	14.14879962	12.8008676
-15	15.59585215	14.83093653	13.56304968
-14	15.25944854	14.26913478	13.21505824
-13	15.8853102	14.69223913	13.47331828
-12	15.98116235	14.7178512	13.56102924
-11	16.18510815	14.63424055	13.81198003
-10	16.55787972	14.86736392	14.03636796
-9	15.73746137	14.50808177	13.63851913
-8	16.69087236	15.0971595	14.82231994
-7	16.34204897	15.03268362	14.77281911
-6	16.9803304	15.49708819	14.79795579
-5	16.89559068	15.25362491	14.09472308
-4	16.60357737	14.9169836	14.20590682
-3	16.48205372	15.1533159	14.45008319
-2	15.89891847	14.56786309	13.8409199
-1	15.52971238	15.14719515	14.3913121
0	11.53666508	14.77192774	13.8589256
1	13.20905633	14.84139529	13.74631566
2	11.47753744	13.88834086	13.02174947
3	11.36676967	13.98496553	13.20881864
4	11.18695032	13.33313525	12.34181127
5	11.39975042	13.48514381	13.25433801
6	11.26402425	13.53060376	13.02121464
7	10.75297124	13.10874733	12.95228191
8	10.56572379	12.79563822	12.55223437
9	10.73841217	12.90117661	12.43510815
10	10.29926313	12.20988828	12.19277395
11	10.01105301	12.23181602	12.17904683
12	9.990016639	12.04973853	11.832541
13	9.296054195	11.19366532	11.03880437
14	9.925124792	11.94342762	11.77787022
15	9.874316615	11.78880437	11.56560494
16	9.653137628	11.73098407	11.46999049
17	9.476230093	11.37051343	11.42756121
18	9.633527454	11.28654623	11.45786784
19	9.585631091	11.45180651	11.40212741
20	9.374019491	11.3531614	11.34252436
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=DarkNetMarkets,
    clip=false,
    width=4cm,
    ymin=0,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}

==> figs/fatpeoplehate/fat_people_hate_active_users.tex <==
\pgfplotstableread{
Week Users Control AskReddit
-20	12052	12124	12080	
-19	12263	12368	12341	
-18	12492	12584	12566	
-17	12673	12773	12730	
-16	12864	12935	12953	
-15	13012	13064	13105	
-14	13170	13262	13303	
-13	13360	13446	13493	
-12	13524	13564	13661	
-11	13550	13591	13752	
-10	13700	13756	13920	
-9	13802	13864	14115	
-8	13918	13978	14299	
-7	13995	14085	14446	
-6	14062	14154	14584	
-5	14050	14222	14707	
-4	13991	14257	14800	
-3	13931	14300	14892	
-2	13691	14290	14916	
-1	12790	14125	14786	
0	12632	14048	14737	
1	12251	13948	14649	
2	12110	13858	14572	
3	11990	13777	14499	
4	11858	13688	14421	
5	11731	13598	14330	
6	11622	13489	14247	
7	11502	13334	14152	
8	11406	13259	14089	
9	11333	13174	14025	
10	11259	13088	13959	
11	11172	13010	13877	
12	11080	12890	13773	
13	11026	12835	13712	
14	10959	12778	13659	
15	10909	12717	13618	
16	10828	12650	13563	
17	10760	12571	13476	
18	10693	12504	13422	
19	10633	12449	13364	
20	10573	12395	13322	
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=FatPeopleHate,
    clip=false,
    width=4cm,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}

==> figs/fatpeoplehate/fat_people_hate_percentage_of_users_gone.tex <==
\begin{tikzpicture}
\begin{axis}[       
        ybar stacked, 
        width=4cm,
        bar width=5pt, 
        title=FatPeopleHate,
        xtick = {1,2,3,4,5,6,7,8,9,10},
        xticklabels = {$2^3$,$2^4$,$2^5$,$2^6$,$2^7$,Control,AskReddit},
        %yticklabels={1,300000}, 
]

%ALL OFF BY 2 FOR LOCATION PURPOSES

%1 week
\addplot+ coordinates
	{
(1,0.0163464295956409)
(2,0.0207526286662976)
(3,0.0358306188925081)
(4,0.0401875418620227)
(5,0.0608324439701174)
(6,0.00711845102505692)
(7,0.00597217509331526)
};


%2 weeks
\addplot+ coordinates
	{
(1,0.0249498135933466)
(2,0.0290536801328168)
(3,0.0504885993485342)
(4,0.0529135967849966)
(5,0.0736392742796158)
(6,0.0135250569476081)
(7,0.011197828299966)
%(9,40)
%(10,6)
};


%3 weeks
\addplot+ coordinates
	{
(1,0.0303986234585603)
(2,0.0392916436081903)
(3,0.0586319218241042)
(4,0.0609511051574012)
(5,0.0917822838847385)
(6,0.0192910022779043)
(7,0.0161520190023752)
%(9, 7)
};


%4 weeks
\addplot+ coordinates
	{
(1,0.0381416690564955)
(2,0.0467625899280575)
(3,0.0688110749185667)
(4,0.0763563295378432)
(5,0.105656350053361)
(6,0.0256264236902049)
(7,0.0214455378350865)
%(9,27)
%(10,3)
};






\end{axis}
\end{tikzpicture}


==> figs/fatpeoplehate/fat_people_hate_week_no_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	25.13587629	23.94641041	22.2333436
-19	25.32387396	23.92919466	22.51170468
-18	24.79700581	24.01709572	22.67706477
-17	24.37323391	23.6428431	21.74444554
-16	24.65710131	23.14307932	21.0200039
-15	24.83412188	23.78943857	21.87664143
-14	24.20910719	22.91449566	21.12501187
-13	24.66943522	23.17377449	21.34321755
-12	24.26518091	23.15990275	21.49227727
-11	24.44251997	22.74755219	21.57104408
-10	24.94279832	23.11205543	21.88492541
-9	23.59707743	22.50156682	20.97121711
-8	24.79904644	23.22894761	22.31836077
-7	24.27219771	22.91394928	22.07004616
-6	24.84091107	23.47088471	22.04497167
-5	24.74921657	23.17933899	20.99176918
-4	24.66063548	22.61264751	21.11624415
-3	24.46502602	23.03314967	21.2650634
-2	23.7629452	22.28820802	20.5265709
-1	23.79224326	23.06342743	21.16931818
0	22.26109391	23.15190463	21.06376445
1	23.63947676	23.82665522	21.29261782
2	22.79254189	22.6422205	20.59686061
3	23.001443	22.98681383	21.11704351
4	22.69761273	22.35206216	20.04710425
5	23.17127672	22.55745527	21.51688211
6	23.46218591	22.93673819	21.21826281
7	22.74396682	22.58333333	21.30189601
8	22.70753512	22.47416762	21.01571983
9	23.42268308	22.79036322	20.96983666
10	22.59955666	21.75185264	20.62110553
11	21.9128512	21.89056684	20.80066985
12	22.11708986	21.86703332	20.40143443
13	21.28064209	20.733847	19.59504219
14	22.26042916	22.10315627	20.73417722
15	22.47903139	21.86991511	20.43532129
16	22.01422957	21.94896598	20.45104895
17	21.96198871	21.40302013	20.47301182
18	22.33884525	21.46829434	20.73035158
19	22.20024773	21.71391549	20.42744597
20	21.84847645	21.64393339	20.48862173

}{\fatpeoplehate}

==> figs/fatpeoplehate/fat_people_hate_week_with_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	14.48882814	13.99387925	12.86991918
-19	14.90117661	14.17863085	13.37217732
-18	14.96101735	14.3591633	13.60785595
-17	14.76182553	14.29135964	13.08569052
-16	15.11397671	14.14879962	12.8008676
-15	15.59585215	14.83093653	13.56304968
-14	15.25944854	14.26913478	13.21505824
-13	15.8853102	14.69223913	13.47331828
-12	15.98116235	14.7178512	13.56102924
-11	16.18510815	14.63424055	13.81198003
-10	16.55787972	14.86736392	14.03636796
-9	15.73746137	14.50808177	13.63851913
-8	16.69087236	15.0971595	14.82231994
-7	16.34204897	15.03268362	14.77281911
-6	16.9803304	15.49708819	14.79795579
-5	16.89559068	15.25362491	14.09472308
-4	16.60357737	14.9169836	14.20590682
-3	16.48205372	15.1533159	14.45008319
-2	15.89891847	14.56786309	13.8409199
-1	15.52971238	15.14719515	14.3913121
0	11.53666508	14.77192774	13.8589256
1	13.20905633	14.84139529	13.74631566
2	11.47753744	13.88834086	13.02174947
3	11.36676967	13.98496553	13.20881864
4	11.18695032	13.33313525	12.34181127
5	11.39975042	13.48514381	13.25433801
6	11.26402425	13.53060376	13.02121464
7	10.75297124	13.10874733	12.95228191
8	10.56572379	12.79563822	12.55223437
9	10.73841217	12.90117661	12.43510815
10	10.29926313	12.20988828	12.19277395
11	10.01105301	12.23181602	12.17904683
12	9.990016639	12.04973853	11.832541
13	9.296054195	11.19366532	11.03880437
14	9.925124792	11.94342762	11.77787022
15	9.874316615	11.78880437	11.56560494
16	9.653137628	11.73098407	11.46999049
17	9.476230093	11.37051343	11.42756121
18	9.633527454	11.28654623	11.45786784
19	9.585631091	11.45180651	11.40212741
20	9.374019491	11.3531614	11.34252436
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=FatPeopleHate,
    clip=false,
    width=4cm,
    ymin=0,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}

==> figs/incels/incels_active_users.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit	
-20	4406	4705	4977	
-19	4455	4756	5039	
-18	4464	4803	5110	
-17	4484	4835	5148	
-16	4530	4880	5199	
-15	4563	4925	5258	
-14	4551	4967	5325	
-13	4581	5009	5370	
-12	4649	5052	5422	
-11	4705	5090	5465	
-10	4745	5130	5509	
-9	4749	5149	5541	
-8	4767	5188	5568	
-7	4755	5217	5587	
-6	4748	5242	5597	
-5	4777	5228	5608	
-4	4817	5234	5642	
-3	4822	5236	5637	
-2	4808	5222	5628	
-1	4730	5199	5611	
0	4570	5156	5571	
1	4515	5115	5533	
2	4467	5084	5500	
3	4426	5057	5467	
4	4366	5004	5436	
5	4331	4976	5403	
6	4304	4945	5375	
7	4266	4914	5344	
8	4213	4857	5310	
9	4181	4822	5276	
10	4155	4788	5248	
11	4125	4755	5218	
12	4097	4720	5195	
13	4065	4684	5167	
14	4046	4654	5145	
15	4009	4620	5114	
16	3981	4581	5093	
17	3928	4532	5056	
18	3899	4497	5031	
19	3874	4463	5009	
20	3840	4432	4977	
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=Incels,
    clip=false,
    width=4cm,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}

==> figs/incels/incels_percentage_of_users_gone.tex <==
\begin{tikzpicture}
\begin{axis}[       
        ybar stacked,
        width=4cm,
        bar width=5pt, 
        title=DarkNetMarkets,
        xtick = {1,2,3,4,5,6,7,8,9,10},
        xticklabels = {$2^3$,$2^4$,$2^5$,$2^6$,$2^7$,Control,AskReddit},
        %yticklabels={1,300000}, 
]

%ALL OFF BY 2 FOR LOCATION PURPOSES

%1 week
\addplot+ coordinates
	{
(1,0.00684931506849317)
(2,0.00813008130081305)
(3,0.0157142857142856)
(4,0.0162412993039443)
(5,0.0366300366300366)
(6,0.00795190069821572)
(7,0.00682103751570628)
};


%2 weeks
\addplot+ coordinates
	{
(1,0.0116438356164383)
(2,0.0199556541019955)
(3,0.0257142857142856)
(4,0.037122969837587)
(5,0.0439560439560439)
(6,0.0139643134212568)
(7,0.0127445700951355)
%(9,40)
%(10,6)
};


%3 weeks
\addplot+ coordinates
	{
(1,0.0157534246575342)
(2,0.0310421286031041)
(3,0.03)
(4,0.0440835266821345)
(5,0.0769230769230768)
(6,0.019200930954228)
(7,0.0186681026745647)
%(9, 7)
};


%4 weeks
\addplot+ coordinates
	{
(1,0.0260273972602739)
(2,0.0376940133037694)
(3,0.0542857142857142)
(4,0.0696055684454756)
(5,0.0915750915750915)
(6,0.0294802172226532)
(7,0.0242326332794829)
%(9,27)
%(10,3)
};






\end{axis}
\end{tikzpicture}

==> figs/incels/incels_week_no_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	32.06123087	27.55993294	27.66684392
-19	31.12061069	28.11187655	27.76906723
-18	28.28831891	27.89489572	27.23775858
-17	29.70849832	28.95726027	26.43198339
-16	30.8386903	29.78282142	25.63911134
-15	30.62104641	30.07246767	26.52277876
-14	29.4013346	30.12746142	25.73801199
-13	31.3412527	28.96157951	25.47861357
-12	32.52680382	28.65304529	26.11293082
-11	33.06638298	29.13852243	25.67018146
-10	31.2743338	29.17978114	25.29908345
-9	30.83450407	29.22265122	25.16893668
-8	32.08427602	29.71106504	24.90313253
-7	31.96165602	28.94821925	24.86250903
-6	29.69605568	30.18128205	24.58026474
-5	30.82824859	29.69885932	25.38626506
-4	30.9713644	29.46625609	25.31054545
-3	32.07201759	29.96990564	24.77882296
-2	33.77956557	29.73878695	24.87720133
-1	33.08974708	29.3857513	25.05107203
0	29.64637343	29.36757751	25.34226406
1	28.51157628	29.50257104	24.23752792
2	27.30293052	28.71020856	24.82770781
3	26.72850832	26.91202673	23.77003573
4	28.48148148	28.53029461	25.63245457
5	27.94236815	28.77465596	24.05179594
6	28.77192362	27.49026346	23.55871608
7	26.65014368	25.77516681	21.6670247
8	26.38833518	24.92376682	20.8518724
9	29.31688596	26.8456276	22.66684783
10	29.67942584	26.42313411	23.50572207
11	28.24298725	27.14456036	23.31346154
12	29.300037	26.93523867	23.0326147
13	30.47297297	27.06447725	23.58594835
14	30.78681733	26.85883785	23.31625835
15	29.48826816	26.48759305	22.56030151
16	30.61590652	26.77952513	23.10576385
17	28.98893974	25.64886681	22.46116505
18	29.59083911	26.34830019	22.53494467
19	30.1283836	26.41193363	23.70974329
20	30.00077791	26.5648855	22.55083767

}{\incels}

==> figs/incels/incels_week_with_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-24	14.85699327	14.61211668	14.36305161
-23	14.51817502	14.55452506	14.01899776
-22	14.74809274	14.65744203	14.55751683
-21	14.31982049	14.75826477	15.02602842
-20	15.35198205	14.75497382	15.56544503
-19	15.2460733	15.26073298	15.63126402
-18	13.69349289	15.20553478	15.56035901
-17	14.58982797	15.81062079	15.23051608
-16	15.35706806	16.39057592	14.84652206
-15	15.4960359	16.69842932	15.76290202
-14	13.8408377	16.93627524	15.41585639
-13	15.1947644	16.23754675	15.50441286
-12	16.79132386	16.46746447	15.9802543
-11	17.43590127	16.51982049	15.65938669
-10	16.67808527	16.75272999	15.69035153
-9	16.41585639	16.98279731	15.75646971
-8	16.97083022	17.15108452	15.45968586
-7	17.20718025	17.14375467	15.44562453
-6	15.31667913	17.60762902	15.2776365
-5	16.32490651	17.52610322	15.75961107
-4	16.5026178	17.17726253	15.61795064
-3	17.45370232	17.57845924	15.36768886
-2	18.84278235	17.45624533	15.63709798
-1	18.20059835	16.96768886	15.555273
0	15.22453254	16.71997008	15.70575916
1	13.44756918	16.30695587	14.60777861
2	12.40373972	15.6499626	14.74435303
3	11.76694091	14.46043381	13.93133882
4	12.53866866	15.35557218	14.98070307
5	11.96694091	15.01361257	13.82303665
6	12.17157816	14.35991025	13.50441286
7	11.09857891	13.29050112	12.07000748
8	10.69349289	12.47120419	11.244727
9	11.9986537	13.50112191	12.47778609
10	12.06267764	13.29259536	12.90441286
11	11.59715782	13.62303665	12.69424084
12	11.84712042	13.25205684	12.46551982
13	12.14360509	13.43709798	12.70501122
14	12.22722513	13.20643231	12.52834705
15	11.84382947	12.77427076	12.08840688
16	12.15018699	12.99117427	12.35302917
17	11.37008227	12.35826477	11.76649215
18	11.49992521	12.28930441	11.57591623
19	11.65474944	12.38219895	12.15811518
20	11.53807031	12.49364248	11.67853403
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=Incels,
    clip=false,
    width=4cm,
    ymin=0,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}

==> figs/missing_data.tex <==
Great Awakening - 7 weeks
Million Dollar Extreme - 7 weeks
Physical Removal - 2 weeks
DarkNetMarkets - 4 weeks
FatPeopleHate - 2 weeks
Incels - 1 week
GunsForSale - 3 weeks
SanctionedSuicide - 2 weeks


==> figs/p_value_data.tex <==
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py Chargers
12.752485263768426 12.752485263768431
1.0
Ttest_indResult(statistic=0.0, pvalue=1.0)
Ttest_relResult(statistic=-8.553104846002448e-17, pvalue=1.0)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py Chargers
14.889515356704477 12.752485263768431
0.0
Ttest_indResult(statistic=4.866675011842748, pvalue=4.448619616477494e-06)
Ttest_relResult(statistic=6.213109803407299, pvalue=1.18392248925206e-07)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py Chargers
14.889515356704477 12.752485263768431
Chargers all users 0.0
Ttest_indResult(statistic=4.866675011842748, pvalue=4.448619616477494e-06)
Ttest_relResult(statistic=6.213109803407299, pvalue=1.18392248925206e-07)
21.379990281102454 19.90591619436475
Chargers no inactives 0.001
Ttest_indResult(statistic=3.763195338767998, pvalue=0.00028877712098567557)
Ttest_relResult(statistic=4.200899767972398, pvalue=0.00011474606804499558)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py darknetmarkets
8.680407006995432 4.340482935383785
darknetmarkets all users 0.0
Ttest_indResult(statistic=24.99678803122381, pvalue=8.180885515398986e-44)
Ttest_relResult(statistic=20.95582818383338, pvalue=8.444867224066953e-26)
21.592773715967486 20.620297706692345
darknetmarkets no inactives 0.0
Ttest_indResult(statistic=4.867834984707127, pvalue=4.4277470705168085e-06)
Ttest_relResult(statistic=4.393858965297283, pvalue=6.127151476040138e-05)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py darknetmarkets_bitcoin_peak
8.294403926252707 4.448637345261768
darknetmarkets_bitcoin_peak all users 0.0
Ttest_indResult(statistic=22.98833544526481, pvalue=8.124492298978981e-41)
Ttest_relResult(statistic=26.137763496989066, pvalue=4.856933354264318e-30)
21.235491383447076 19.836527205883726
darknetmarkets_bitcoin_peak no inactives 0.0
Ttest_indResult(statistic=7.49444910905461, pvalue=3.284625365018148e-11)
Ttest_relResult(statistic=7.096930494774141, pvalue=5.223295377639975e-09)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py fatpeoplehate
12.757904706926745 9.259230243083682
fatpeoplehate all users 0.0
Ttest_indResult(statistic=7.758418671363113, pvalue=9.187143219649935e-12)
Ttest_relResult(statistic=12.686289528419094, pvalue=6.058371115397813e-17)
24.12289431148003 21.71835451037981
fatpeoplehate no inactives 0.0
Ttest_indResult(statistic=15.107302443253046, pvalue=4.09351766633274e-27)
Ttest_relResult(statistic=18.57641785458421, pvalue=1.473320273652309e-23)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py greatawakening
12.889814703001512 7.6012988232768475
greatawakening all users 0.0
Ttest_indResult(statistic=8.292855216942694, pvalue=6.793776304356274e-13)
Ttest_relResult(statistic=10.43935237477167, pvalue=6.082452656749853e-14)
27.970940982416653 24.335196509507156
greatawakening no inactives 0.0
Ttest_indResult(statistic=3.9405173548370698, pvalue=0.00015430527083119255)
Ttest_relResult(statistic=3.523404152980495, pvalue=0.0009466816807694737)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py gunsforsale
15.732378335949768 13.763500784929354
gunsforsale all users 0.0
Ttest_indResult(statistic=7.575006414760231, pvalue=2.2287942058548525e-11)
Ttest_relResult(statistic=8.94392928178172, pvalue=8.576361624332105e-12)
21.67493690687381 21.689685488200407
gunsforsale no inactives 0.955
Ttest_indResult(statistic=-0.046781927862452034, pvalue=0.9627842150275234)
Ttest_relResult(statistic=-0.049848373654182085, pvalue=0.9604500722131558)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py incels
14.801553890067622 11.142350373208373
incels all users 0.0
Ttest_indResult(statistic=13.849884573522775, pvalue=1.2789677575651177e-24)
Ttest_relResult(statistic=21.163176405193248, pvalue=5.507946036721408e-26)
31.573177724432227 29.51190606806681
incels no inactives 0.0
Ttest_indResult(statistic=6.5492096743730395, pvalue=2.8569036660227662e-09)
Ttest_relResult(statistic=5.3951770113868704, pvalue=2.073368115361662e-06)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py milliondollarextreme
15.906633686560378 7.5570457082225175
milliondollarextreme all users 0.0
Ttest_indResult(statistic=16.398819239690308, pvalue=1.373570180712935e-29)
Ttest_relResult(statistic=16.60525559721923, pvalue=1.5763786820436216e-21)
26.065664182078372 19.654059347603233
milliondollarextreme no inactives 0.0
Ttest_indResult(statistic=8.672234935831465, pvalue=1.0537146883508988e-13)
Ttest_relResult(statistic=9.03865918796698, pvalue=6.221488429524987e-12)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py physical_removal
37.35990646258504 24.735260770975056
physical_removal all users 0.0
Ttest_indResult(statistic=8.991374536839997, pvalue=2.1833117929806835e-14)
Ttest_relResult(statistic=11.205777029024572, pvalue=5.352073342592444e-15)
55.1749849124539 47.015531816555004
physical_removal no inactives 0.0
Ttest_indResult(statistic=8.53467551255823, pvalue=2.073399176016279e-13)
Ttest_relResult(statistic=7.912095581007262, pvalue=2.990628873695991e-10)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py sanctionedsuicide
11.837210531881146 7.429724013957914
sanctionedsuicide all users 0.0
Ttest_indResult(statistic=14.741214443007966, pvalue=2.1373708674739426e-26)
Ttest_relResult(statistic=20.093950970854618, pvalue=5.17925644165321e-25)
28.692183641640195 25.904037947607893
sanctionedsuicide no inactives 0.0
Ttest_indResult(statistic=5.829543322266399, pvalue=7.440740152876932e-08)
Ttest_relResult(statistic=6.09226199612568, pvalue=1.8123261634001126e-07)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py SandersForPresident
19.87935331798674 15.631145967559648
SandersForPresident all users 0.0
Ttest_indResult(statistic=9.249638873449442, pvalue=6.091777500669883e-15)
Ttest_relResult(statistic=13.14475055383758, pvalue=1.6012277285202984e-17)
27.917956018006844 25.769494761057047
SandersForPresident no inactives 0.0
Ttest_indResult(statistic=6.452738697591108, pvalue=4.458757848874061e-09)
Ttest_relResult(statistic=7.982590946009462, pvalue=2.339610700451842e-10)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py StarWars_lastjedi
25.52023535097208 21.43727933297513
StarWars_lastjedi all users 0.0
Ttest_indResult(statistic=15.430348072185007, pvalue=9.65348796602807e-28)
Ttest_relResult(statistic=14.863475163657586, pvalue=1.3759613839075525e-19)
31.606603900854044 29.04068443827767
StarWars_lastjedi no inactives 0.0
Ttest_indResult(statistic=11.698295237485125, pvalue=3.559446927262422e-20)
Ttest_relResult(statistic=10.755477864533585, pvalue=2.2119045183715342e-14)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py StLouisRams
20.24207525333785 15.188330934033367
StLouisRams all users 0.0
Ttest_indResult(statistic=9.101854628535124, pvalue=1.2649200679283238e-14)
Ttest_relResult(statistic=9.642675556533565, pvalue=8.222118229832279e-13)
27.76323433474474 22.92545528852479
StLouisRams no inactives 0.0
Ttest_indResult(statistic=8.920779681453883, pvalue=3.093818288942368e-14)
Ttest_relResult(statistic=8.241420227452192, pvalue=9.529963002930008e-11)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py the_donald_election
13.941715877689369 11.879731134554348
the_donald_election all users 0.0
Ttest_indResult(statistic=4.410424877015568, pvalue=2.694644998913201e-05)
Ttest_relResult(statistic=8.117257154013837, pvalue=1.465270455028683e-10)
23.83456446440088 22.291468382306597
the_donald_election no inactives 0.0
Ttest_indResult(statistic=4.774483491504347, pvalue=6.4523138555653225e-06)
Ttest_relResult(statistic=5.319511443466002, pvalue=2.6935782866411613e-06)
(env) pthomas4@dsg2:/data/pthomas4/wordAdoption python3 p_tests.py the_donald_rnc
16.613688912319105 15.122251287149707
the_donald_rnc all users 0.028
Ttest_indResult(statistic=2.205827689564352, pvalue=0.029782039199935884)
Ttest_relResult(statistic=4.701513584867855, pvalue=2.2100774808110115e-05)
26.684043847507485 25.830696332969065
the_donald_rnc no inactives 0.055
Ttest_indResult(statistic=2.0861067189495843, pvalue=0.03962057973488021)
Ttest_relResult(statistic=3.0483397599585085, pvalue=0.0037363914666172014)


==> figs/physical_removal/physical_removal_active_users.tex <==
\pgfplotstableread{
Week Users Control AskReddit
-20 475 478 481
-19 480 480 483
-18 486 484 492
-17 491 486 498
-16 495 491 497
-15 496 491 499
-14 494 489 508
-13 494 491 507
-12 496 497 513
-11 502 501 515
-10 506 503 515
-9 507 503 521
-8 504 507 521
-7 509 511 521
-6 508 516 520
-5 502 518 522
-4 501 518 522
-3 493 517 521
-2 477 511 518
-1 469 510 516
0 463 509 514
1 457 508 511
2 451 505 509
3 445 502 506
4 443 500 506
5 438 493 506
6 433 489 505
7 427 486 501
8 422 484 500
9 418 482 499
10 416 481 498
11 413 479 496
12 412 475 496
13 409 473 494
14 406 472 492
15 405 472 491
16 403 470 489
17 401 468 486
18 397 463 486
19 395 461 485
20 390 456 479
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=Physical\textunderscore Removal,
    clip=false,
    width=4cm,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}

==> figs/physical_removal/physical_removal_no_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	61.09839817	51.29655172	42.91294118
-19	59.92201835	57.69614512	37.79058824
-18	62.08333333	55.02036199	38.13785047
-17	62.51801802	59.66219239	41.96766744
-16	67.30634573	58.37555556	40.55
-15	61.88962472	62.40748899	36.99300699
-14	62.32251082	60.09713024	36.7
-13	60.42666667	55.04861111	36.02588235
-12	59.64782609	56.62837838	38.60046729
-11	58.4463895	57.17943107	35.94158879
-10	59.31372549	56.46799117	36.86574074
-9	56.36323851	61.72828508	36.22068966
-8	55.33406593	55.38189845	36.58796296
-7	59.10217391	60.48017621	37.96018735
-6	57.8722467	57.56017505	39.47191011
-5	56.39867841	54.55482456	36.11600928
-4	54.92650334	55.56652361	37.42237443
-3	54.5862069	57.30973451	37.4562212
-2	54.0046729	53.15536105	36.54462243
-1	47.71212121	54.8185941	36.01366743
0	51.24438903	56.29820628	34.79398148
1	53.51530612	57.82783019	36.78846154
2	48.55526316	54.77931034	36.68585132
3	45.94623656	52.55244755	35.45673077
4	43.83870968	49.70518868	34.36567164
5	42.82887701	49.41866029	35.58088235
6	45.36712329	48.11835749	34.49156627
7	48.26256983	54.13868613	32.39320388
8	45.92329545	50.14841849	34.03274559
9	42.42363112	51.24205379	31.88148148
10	44.46802326	52.51932367	33.6019656
11	45.98809524	53.60493827	34.69
12	48.375	53.2962963	35.67183463
13	45.41411043	51.7755611	32.60651629
14	45.52795031	58.10831234	35.41025641
15	45.2672956	52.60305344	34.09974425
16	47.69631902	55.7755611	36.2761194
17	47.47515528	49.42893401	33.67493797
18	51.63322884	53.53117207	34.82531646
19	44.37699681	47.35897436	30.73629243
20	45.80655738	46.96276596	30.10103627


}{\physicalremoval}

==> figs/physical_removal/physical_removal_week_with_inactives.tex <==
\pgfplotstableread{
Week	Users	Control	AskReddit
-20	46.35416667	38.73958333	31.66319444
-19	45.35763889	44.17361111	27.88368056
-18	47.85590278	42.22048611	28.33854167
-17	48.19097222	46.30034722	31.54861111
-16	53.40104167	45.60590278	29.56770833
-15	48.67361111	49.18923611	27.55208333
-14	49.98784722	47.26388889	26.76041667
-13	47.20833333	41.28645833	26.58159722
-12	47.63541667	43.65104167	28.68229167
-11	46.37152778	45.36631944	26.70659722
-10	47.265625	44.40972222	27.64930556
-9	44.71875	48.11805556	27.35416667
-8	43.71006944	43.55555556	27.44097222
-7	47.19965278	47.67013889	28.140625
-6	45.61458333	45.66840278	30.49479167
-5	44.453125	43.18923611	27.02430556
-4	42.81597222	44.95486111	28.45659722
-3	41.22395833	44.97222222	28.22222222
-2	40.12847222	42.17361111	27.72569444
-1	32.80208333	41.97048611	27.44791667
0	35.67534722	43.59201389	26.09548611
1	36.42013889	42.56770833	26.56944444
2	32.03298611	41.36979167	26.55902778
3	29.67361111	39.140625	25.60763889
4	28.3125	36.58854167	23.984375
5	27.80902778	35.86284722	25.203125
6	28.74826389	34.58506944	24.85069444
7	29.99652778	38.63020833	23.17013889
8	28.06423611	35.78298611	23.45659722
9	25.55729167	36.38541667	22.41666667
10	26.55729167	37.74826389	23.74305556
11	26.82638889	37.69097222	24.09027778
12	26.875	37.47395833	23.96701389
13	25.703125	36.04513889	22.58680556
14	25.45138889	40.05034722	23.97569444
15	24.99131944	35.890625	23.14756944
16	26.99479167	38.82986111	25.31770833
17	26.53993056	33.81076389	23.56076389
18	28.59548611	37.26736111	23.88194444
19	24.11458333	32.06597222	20.4375
20	24.25520833	30.65625	20.171875
}{\adoptions}
\begin{tikzpicture}
    \begin{axis}[
    title=Physical\textunderscore Removal,
    clip=false,
    width=4cm,
    ymin=0,
    ]
    \addplot [mark=*, blue, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Users]   {\adoptions};
    \addplot [mark=*, red, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=Control]   {\adoptions};
    \addplot [mark=*, orange, mark size=0.75pt, fill opacity=0.5, draw opacity=0.2]  table [x=Week, y=AskReddit]   {\adoptions};
    \end{axis}
\end{tikzpicture}
